Exploring the Environmental Benefits of In-Process Isolation for Software Resilience

Memory-related errors remain an important cause of software vulnerabilities. While mitigation techniques such as using memory-safe languages are promising solutions, these do not address software resilience and availability. In this paper, we propose a solution to build resilience against memory attacks into software, which contributes to environmental sustainability and security.

==> Makefile <==

ISPELLPAT = -ktexskip1 +cref,Cref,url,todo,presetkeys,newcommand,definecolor


all: main.pdf

main.pdf: *.tex sections/*.tex *.bib
	latexmk -pdflatex='pdflatex -file-line-error' -pdf main.tex
	$(MAKE) wordcount

wordcount: abstract.tex
	@echo === abstract: 150 ===
	wc -w abstract.tex
	@echo ===

spelling: *.tex sections/*.tex
	for file in *.tex sections/*.tex; do \
          ispell -t ${ISPELLPAT} -b -d american -p ./paper.dict $$file; \
        done

clean:
	latexmk -C -pdflatex='pdflatex -file-line-error' -pdf main.tex
	rm -f main.pdf
	rm -f *.tex.bak

distclean: clean
	rm -f main.bbl


